Novel Demonstration Generation with Gaussian Splatting Enables Robust One-Shot Manipulation

Visuomotor policies learned from teleoperated demonstrations face challenges such as lengthy data collection, high costs, and limited data diversity. Existing approaches address these issues by augmenting image observations in RGB space or employing Real-to-Sim-to-Real pipelines based on physical simulators. However, the former is constrained to 2D data augmentation, while the latter suffers from imprecise physical simulation caused by inaccurate geometric reconstruction. This paper introduces RoboSplat, a novel method that generates diverse, visually realistic demonstrations by directly manipulating 3D Gaussians. Specifically, we reconstruct the scene through 3D Gaussian Splatting (3DGS), directly edit the reconstructed scene, and augment data across six types of generalization with five techniques: 3D Gaussian replacement for varying object types, scene appearance, and robot embodiments; equivariant transformations for different object poses; visual attribute editing for various lighting conditions; novel view synthesis for new camera perspectives; and 3D content generation for diverse object types. Comprehensive real-world experiments demonstrate that RoboSplat significantly enhances the generalization of visuomotor policies under diverse disturbances. Notably, while policies trained on hundreds of real-world demonstrations with additional 2D data augmentation achieve an average success rate of 57.2%, RoboSplat attains 87.8% in one-shot settings across six types of generalization in the real world.

==> table/exp_appearance.tex <==
\begin{tabular}{cccc}
\toprule
 & Pick object & Close drawer & Pick-Place-Close \\
\midrule
collected & 3/30 & 0/30 & 0/30 \\
augmented w/o appearance augmentation 200 & 0/30 & 1/30 & 0/30 \\
augmented w/o appearance augmentation 1800 & 5/30 & 4/30 & 3/30 \\
augmented with appearance augmentation 3200 & 30/30 & 28/30 & 25/30 \\
\bottomrule
\end{tabular}


==> table/exp_embodiment.tex <==
\begin{tabular}{cccc}
\toprule
 & Pick object & Close drawer & Pick-Place-Close \\
\midrule
collected & 0 & 0 &  \\
augmented w/o embodiment augmentation & 0 & 0 &  \\
augmented with embodiment augmentation & 30/30 & 29/30 &  \\
\bottomrule
\end{tabular}


==> table/exp_lighting.tex <==
\begin{tabular}{cccc}
\toprule
 & Pick object & Close drawer & Pick-Place-Close \\
\midrule
collected & 3/30 & 5/30 & 3/30 \\
augmented w/o lighting augmentation 200 & 7/30 & 5/30 & 3/30 \\
augmented w/o lighting augmentation 1800 & 5/30 & 15/30 & 3/30 \\
augmented with lighting augmentation 3200 & 24/30 & 28/30 & 24/30 \\
\bottomrule
\end{tabular}


==> table/exp_main.tex <==
\begin{tabular}{ccccc}
\toprule
 & Pick object & Close drawer & Pick-place-close & Long pick 2\\
\midrule
100 collected demos & 18/30 & 29/30 & 4/30 & 19/30 \\
200 collected demos & 28/30 & \textbf{30/30} & 23/30 & 24/30 \\
100 augmented demos & 15/30 & 27/30 & 4/30 & 0/30 \\
200 augmented demos & 24/30 & 28/30 & 17/30 & 13/30\\
800 augmented demos & 28/30 & \textbf{30/30} & 22/30 & 25/30 \\
1800 augmented demos & \textbf{30/30} & - & \textbf{25/30} & \textbf{29/30} \\
\bottomrule
\end{tabular}


==> table/exp_object.tex <==
\begin{tabular}{ccc}
\toprule
 & Novel category \\
\midrule
collected & 7/30 \\
augmented w/o object augmentation 1600 & 10/30 \\
augmented with object augmentation 6400 & 23/30 \\
\bottomrule
\end{tabular}

